Auto-FedRL: Federated Hyperparameter Optimization for Multi-institutional Medical Image Segmentation

Federated learning (FL) is a distributed machine learning technique that enables collaborative model training while avoiding explicit data sharing. The inherent privacy-preserving property of FL algorithms makes them especially attractive to the medical field. However, in case of heterogeneous client data distributions, standard FL methods are unstable and require intensive hyperparameter tuning to achieve optimal performance. Conventional hyperparameter optimization algorithms are impractical in real-world FL applications as they involve numerous training trials, which are often not affordable with limited compute budgets. In this work, we propose an efficient reinforcement learning (RL)-based federated hyperparameter optimization algorithm, termed Auto-FedRL, in which an online RL agent can dynamically adjust hyperparameters of each client based on the current training progress. Extensive experiments are conducted to investigate different search strategies and RL agents. The effectiveness of the proposed method is validated on a heterogeneous data split of the CIFAR-10 dataset as well as two real-world medical image segmentation datasets for COVID-19 lesion segmentation in chest CT and pancreas segmentation in abdominal CT.

==> algorithms/auto_fedrl.tex <==
\begin{algorithm}[]
\SetAlgoNoLine
\SetArgSty{textnormal}
\textbf{Input}: initial global model $\Theta^1$; initial hyperparameter combination $h^1$; server optimizer {\tt ServerOpt}; client optimizer {\tt ClientOpt}; RL optimizer {\tt RLOpt}; RL learning rate $\gamma_h$ . \\ 
	\For{q = 1 to Q}{
		\For{k = 1 to K \textbf{in parallel}} {
			$\triangleright$ \text{deploy $h^q$ to clients} \\
			\If{q = 1}{
			$\triangleright$ \text{deploy $\Theta^{q}$ to clients}}
			$\triangleright$ \text{unpack $P^q$ and $\gamma_k^q$,  from $h^q$} \\
			$\Theta^{q}_k \leftarrow$ {\tt LocalTrain} ($\Theta^{q},P^q,\gamma_k^q$) \\
			
			$\triangleright$  $\Delta_k^q = \Theta^{q}-\Theta^{q}_k$ \\
			$\triangleright$ \text{upload $\Delta_k^q$ to the server} \\
		}
		$\triangleright$ \text{unpack $\alpha_k^q$ and $\gamma^q$,  from $h^q$}
	
	    $\triangleright$ $\Delta^q = \sum\limits_{k=1}^{K} \alpha_k^q \Delta_k^q$ \\
		$\Theta^{q+1}$ $\leftarrow$ {\tt ServerOpt}( $\Theta^{q}$,$-\Delta^q$,$\gamma^q$) \\
		$h^{q+1} $ $ \leftarrow$ {\tt RLUpdate}( $\Theta^{q+1}$,$\gamma_h$) \\
	}
	\Return{$\Theta^Q$}\\
	{\tt LocalTrain($\Theta^{q},P^q,\gamma_k^q$)}:\\
	\Indp$\Theta^{q,1}_{k} \leftarrow \Theta^{q}$ \\
	\For{p = 1 to P}{
		$\triangleright$ compute the gradients $g_{k}^{q,p}$ \\
		$\triangleright$ $\Theta^{q,p+1}_{k}$ =  {\tt ClientOpt}( $\Theta^{q,p}_{k}$,$g_{k}^{q,p}$,$\gamma_k$) \\
			}
    \Return{$\Theta^{q}_{k}$}	\\		
	\Indm {\tt RLUpdate} ($\Theta^{q+1}$,$\gamma_h$):\\
	\Indp $\triangleright$ \text{deploy $\Theta^{q+1}$ to clients} \\
	\For{k = 1 to K $\textbf{in parallel}$}{
		$\triangleright$ compute and upload $\mathcal{L}_{\text{val}_{k}}^{q+1}$  to the server \\
			}
	$\mathcal{L}_h^{q+1}=\frac{1}{K}\sum\limits_{k=1}^{K}\mathcal{L}_{\text{val}_{k}}^{q+1}$\\
	$\triangleright$ Compute $r^q$ with Eq.~\ref{eq:4} \\
	$\psi^{q+1} \leftarrow$ {\tt RLOpt}($r^{q+1}$,$\gamma_h$) with Eq.~\ref{eq:7}\\
	$h^{q+1} \sim P(\mathcal{H}| \psi^{q+1})$ \\
	\Return{$h^{q+1}$}\\
	
 \caption{Auto-FedRL}\label{al:2}
\end{algorithm}

==> algorithms/fedopt.tex <==
\begin{algorithm}[t!]
\SetAlgoNoLine
\small
\caption{Adaptive Federated Optimization}\label{al:1}
\textbf{Input}: initial global model $\Theta^0$; server learning rate $\gamma$; client learning rate $\gamma_k$; server optimizer {\tt ServerOpt}, client optimizer {\tt ClientOpt}. \\ 
	\For{q = 1 to Q}{
		\For{k = 1 to K \textbf{in parallel}} {
			$\triangleright$ \text{deploy weights to local models} \\
			\For{p = 1 to P}{
				$\triangleright$ compute the gradients $g_{k}^{q,p}$ \\
				$\triangleright$ $\Theta^{q,p+1}_{k}$ =  {\tt ClientOpt}( $\Theta^{q,p}_{k}$,$g_{k}^{q,p}$,$\gamma_k$) \\
			}
			$\triangleright$ \text{upload weights to the server} \\
			$\triangleright$  $\Delta_k^q = \Theta^{q}-\Theta^{q}_k$
		}
		$\triangleright$ $\Delta^q = \sum\limits_{k=1}^{K} \alpha_k \Delta_k^q$ \\
		$\triangleright$ $\Theta^{q+1}$ =  {\tt ServerOpt}( $\Theta^{q}$,$-\Delta^q$,$\gamma$) \\
	}
	\Return{$\Theta^Q$}
	%\vskip-10pt
\end{algorithm}

==> tables/add_cifar_comput.tex <==
\begin{table}[t!]
	\setlength{\tabcolsep}{2.0pt}
	%\scriptsize
	\caption{The additional computational details of different search strategies under the same setting on CIFAR-10.}\label{tb5}
	\centering
	\vskip-8pt
%\resizebox{0.475\textwidth}{!}{
\begin{tabular}{l|cccc}
\hline
Search Space Type & Accuracy &Memory Usage & Running Time for Search & C3-Score~\cite{c3} \\\hline\hline
Discrete &    90.70 & 42.8 GB     & 8.246 s  &  0.778    \\
Continuous &  90.85 & \redbf{3.00 GB}      & \redbf{0.012 s}  & \blueud{0.799}           \\ 
Continuous MLP &  91.27 & \blueud{3.13 GB}      & \blueud{0.019 s}   & \redbf{0.803}        \\ \hline
\end{tabular}
%}
\vskip-10pt
\end{table}
